Visual Data Diagnosis and Debiasing with Concept Graphs

The widespread success of deep learning models today is owed to the curation of extensive datasets significant in size and complexity. However, such models frequently pick up inherent biases in the data during the training process, leading to unreliable predictions. Diagnosing and debiasing datasets is thus a necessity to ensure reliable model performance. In this paper, we present ConBias, a novel framework for diagnosing and mitigating Concept co-occurrence Biases in visual datasets. ConBias represents visual datasets as knowledge graphs of concepts, enabling meticulous analysis of spurious concept co-occurrences to uncover concept imbalances across the whole dataset. Moreover, we show that by employing a novel clique-based concept balancing strategy, we can mitigate these imbalances, leading to enhanced performance on downstream tasks. Extensive experiments show that data augmentation based on a balanced concept distribution augmented by Conbias improves generalization performance across multiple datasets compared to state-of-the-art methods.

==> main_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    Table 1 in the main paper and our extended analysis section demonstrate the usefulness of our approach.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss limitations of our work in the final section of the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There are no theoretical results or proofs in the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include details of the datasets in both the main paper and supplementary. The implementation of baselines rely on open source codes that are well documented. Further, we will release our own code for better reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We attach the code in addition to the supplementary material. All datasets except UrbanCars are open source. The code to generate UrbanCars, however, is open source.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All training details and hyperparameters are included in the main paper as well as the supplementary.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All results reported are the mean of three separate training runs. We include error bars in the supplementary material, and omit them from Table 1 in the main paper for better readability.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide details on the architecture used and the time of execution in the supplementary.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have reviewed and agree to the NeurIPS code of ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the broader impact of our work in the supplementary.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We perform the necessary manual checks to ensure the safety of our data generation process. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All original creators/owners of assets are cited in the work. We use CC-BY 4.0 license.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We share the code to reproduce experiments in our work, and will make them open source.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work does not involve research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work does not involve research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> section/exp_bk.tex <==
\section{Experiments}
\label{s_exp}

We validate \ourmethod

We begin by introducing the experimental setup including the datasets, baselines, implementation details in Section~\re{s_exp_setup}, following by our main results across various types of datasets in Section~\ref{d}

% We begin by outlining the tasks we solve in this paper, the datasets, the baselines, implementation details, and finally we present our main results.

\subsection{Setup}\label{s_exp_setup}
% We begin by outlining the tasks we solve in this paper, the datasets, the baselines, implementation details, and finally we present our main results.
\mypara{Datasets.}
We use three datasets in our work: Waterbirds, UrbanCars, and COCO-GB. We tackle background bias in the Waterbirds dataset, background and co-occuring object bias in the UrbanCars dataset, and finally gender bias in COCO-GB. All the tasks are binary classification tasks. More details on the training splits and class labels are provided in the Appendix. 

\mypara{Baseline methods.}
Our baselines are include a vanilla Resnet-50 model pre-trained on ImageNet, two typical data augmentation based debiasing methods - (1) CutMix, a technique where we cut and paste patches between different training images to generate diverse discriminative features, and (2) RandAug, which creates random transformations on the training data during the learning phase. Finally, we compare against the recently proposed and state-of-the-art ALIA\cite{dunlap2024diversify}, which uses a large language model to generate diverse, in-distribution prompts for a text-to-image generative model.

\mypara{Evaluation}

We compute the mean test accuracy over the class-balanced test data and the out-of-distribution (OOD) test data, similar to \cite{dunlap2024diversify}. The class-balanced data contains an even distribution of classes and their respective spurious correlations, while the OOD data contains counterfactual concepts. For example, in  Waterbirds dataset, for the class-balanced test data 50\%\ images of Landbirds have Land backgrounds, while 50\%\ images of Waterbirds have Water backgrounds. The OOD test set contains Landbirds on Water, and Waterbirds on Land. More details on the test sets are presented in the Appendix.

\mypara{Implementation details.}
We use existing implementations to train our models. Our Base model is a Resnet-50 pretrained on ImageNet. We generate the same number of images per data-augmentation protocol to ensure a fair comparison. For comparison with ALIA on Waterbirds, we directly use their generated dataset available here. For the other datasets, we used the existing ALIA implementation to generate the augmented data. We use validation loss based checkpointing to choose the best model, the ADAM optimizer with a learning rate of $1e-3$, a weight decay of $1e-5$, and a cosine learning schedule over $100$ epochs. This is all following previous work, to ensure a fair comparison. To generate images, we use Stable Diffusion inpainting with a CLIP-based filtering mechanism to ensure reliable image generation. This is similar to the process in \cite{dunlap2024diversify}. While the authors experimented with a variety of text-to-image generative models, we found satisfactory results with our generation protocol. Our core contribution lies in the bias diagnosis and mitigation, not in proposing a new generative process. More details on the generative model hyperparameters are presented in the Appendix.
\subsection{Main Results}
%%%%%%%%%%%%%%%%%
\input{table/main_results}
%%%%%%%%%%%%%%%%%

% \begin{table}[h]
% \centering
% \caption{Mean Test Accuracy on different datasets. Results are averaged over three training runs.}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Method} & \multicolumn{2}{c}{\textbf{Waterbirds}} & \multicolumn{2}{c}{\textbf{UrbanCars}} & \multicolumn{2}{c}{\textbf{COCO-GB}} \\
%  & \textbf{Class Balanced} & \textbf{OOD} & \textbf{Class Balanced} & \textbf{OOD} & \textbf{Class Balanced} & \textbf{OOD} \\
% \midrule
% Base & 67.05 & 44.93 & 84.37 & 44.53 & & \\
% Base (+RandAug) & 73.66 & 60.22 & 87.73 & 56.00 & & \\
% Base (+ALIA) & 69.57 & 48.17 & & & & \\
% Base (+Ours) & \textbf{77.9} & \textbf{69.26} & & & & \\
% \bottomrule
% \end{tabular}
% \end{table}

In Table \ref{tab:main} we present the main results, averaged over three training runs. 

First, we note that for Waterbirds and UrbanCars, we observe significant improvements in both the Class-Balanced and OOD test sets over the typical augmentation methods such as CutMix and RandAug. 

Second, we note the significant improvement in performance over the most recent state-of-the-art augmentation method, ALIA. 

Third, for COCO-GB, while we notice slightly smaller difference in the CB and OOD accuracies between our method and the baselines, our hypothesis is that this happens because of limited number of samples used for augmentation. ALIA uses a confidence based filtering mechanism to remove generated samples. This leads to a small final number of 260 samples to be added for the retraining part. In the ablation section, we show this hypothesis to be true, and further demonstrate that on adding more images for the retraining step, we progressively increase the performance gap between our method and the baselines. These three observations taken together validate the usefulness of our approach. The next section provides additional insights on the usefulness of our method and the effect of ablating its components.
\subsection{Ablations and Analyses}
% \begin{itemize}

%     \item Note on the imbalance I and the number of upsampled images. 
    
%     \item "Good" bias and "Bad" bias: What features constitute bias? What features do not?

%     \item Use of graph structure: Add baseline results if only using 1-hop neighborhood sampling. Here we show that cliques are useful. 

%     \item Assuming access to a small test set to check for relevant concepts. 

%     \item Maybe some comments on size of cliques?

%     \item Note on class-imbalance and long-tail?

%     \item Replace generative model with InstructPix2Pix and Waterbirds prompts from ALIA. 
% \end{itemize}
In this section, we further analyze our method along four axes: (i) The usefulness of the graph clique approach, (ii) The alignment between the discovered concepts by our method and the trained classifier attributions, (iii) The impact of the generative component in our work compared to ALIA, since the latter uses InstructPix2Pix while we use a stable diffusion based inpainting protocol, and (iv) The impact on CB and OOD performance by increasing the number of added samples for the retraining step.


\subsubsection{The use of the graph structure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\linewidth]{NeurIPS 2024/figure/graph_structure.png}
    \caption{Leveraging the graph structure improves generalization performance. Results on UrbanCars which has two shortcuts: Background and Co-Occurring object. Results averaged over three training runs. \Cheng{do the table, leave it there.}}
    \label{fig:graph}
\end{figure}
Recalling the definition of Class Clique Sets, in principle one could only use cliques sizes of 1, i.e. the direct neighbors of each class node. This would be equivalent to computing the frequency of co-occurrence over a single hop neighborhood. In this ablation we show that one should use larger cliques, i.e. leverage the graph structure, instead of a simple direct neighborhood based frequency calculation. We trained three separate models on three different types of $D_{aug}$: Ours(BG), trained on images containing only background shortcuts, Ours(CoObj), images containing only the co-occurrence shortcuts, and Ours(Both), images containing both shortcuts, but \textit{not simultaneously}. Figure \ref{fig:graph} validates the use of the concept graph. 

First, our approach of leveraging the graph structure provides improvement over simply using the frequency of a 1-hop neighborhood. 

Second, we note that \textit{all} the methods outperform the baseline and ALIA, which shows that incorporating frequency based co-occurrences is in a broader sense much more useful than relying on diverse prompts generated by ChatGPT-4, which is the approach taken by ALIA.

\subsubsection{Robustness to evaluation metrics}

The CB and OOD test accuracies test for generalization capabilities, but more direct evaluators of shortcut learning exist in the literature. In \cite{li2023whac}, for instance, the authors propose (i) The \textbf{ID Accuracy} -  which is the accuracy when the test set contains common background and co-occurring objects, (ii) The \textbf{BG-GAP} -  which is the drop in \textbf{ID accuracy} when the test set contains common co-occurring objects, but uncommon background objects, (iii) The \textbf{CoObj-GAP},  which is the drop in \textbf{ID accuracy} when the test set contains uncommon co-occurring objects, but common background objects, and finally (iv) The \textbf{BG + CoObj GAP}, which is the case when both background and co-occurring objects are uncommon in the test set. A multiple shortcut mitigation method should \textit{minimize} the \textbf{BG + CoOBj GAP} metric, and also make sure it does not exacerbate any shortcut that the base model relies on. In short, the method should also reduce the \textbf{BG-GAP} and \textbf{CoObj-GAP} when compared to the base model. In Table \ref{tab:gaps}, we present results of Base, Base + Ours(BG), Base + Ours(CoObj), Base + Ours(Both), and Base + Ours on these metrics.  

\input{NeurIPS 2024/table/coobj_bg_gap}
First we note the \textbf{BG+CoObj GAP}, which evaluates how well the model mitigates multiple shortcuts. Here, we see that by using the graph approach, where we compute multiple concept co-occurrences with the classes, instead of single concept co-occurrences, we have the smallest drop from the \textbf{ID accuracy}, which is what is desired. Second, we note that our model posts the smallest drop in the \textbf{CoObj-GAP} metric as well, which suggests the mitigation of the co-occurring object shortcut. Third, we notice that \textit{Base(BG)} posts the smallest drop in background reliance, which suggests an interesting idea, that not all shortcuts in a dataset are created the same, i.e. it is possible the background may be the higher priority shortcut to mitigate, instead of the co-occurring object. It will be an interesting point of future work to incorporate this idea into our framework. Overall, we are able to show that indeed, use of multiple node cliques mitigates mutiple shortcuts better than single class-concept frequency imbalances. This places our method in a more realistic context, as it is infeasible to assume that real world data will only have a single type of bias in them.

\subsubsection{Discovered concept imbalances and feature attributions}

% \begin{figure}[t]
% \centering
% % Row 1
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch24_image7_base.png}
% \end{minipage}%
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch33_image6_base.png}
% \end{minipage}%
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch52_image2_base.png}
% \end{minipage}
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch53_image6_base.png}
% \end{minipage}
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch89_image6_base.png}
% \end{minipage}

% %Row 2
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch24_image7_alia.png}
% \end{minipage}%
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch33_image6_alia.png}
% \end{minipage}%
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch52_image2_alia.png}
% \end{minipage}
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch53_image6_alia.png}
% \end{minipage}
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch89_image6_alia.png}
% \end{minipage}
% \\
% %%Row 3

% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch24_image7_conbias.png}
% \end{minipage}%
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch33_image6_conbias.png}
% \end{minipage}%
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch52_image2_conbias.png}
% \end{minipage}
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch53_image6_conbias.png}
% \end{minipage}
% \begin{minipage}{0.15\textwidth}
%     \includegraphics[width=0.7\linewidth]{NeurIPS 2024/figure/heatmap_batch89_image6_conbias.png}
% \end{minipage}

% % Add additional rows following the same pattern
% % Row 3
% \begin{minipage}{0.33\textwidth}
%     \includegraphics[width=\linewidth]{image4.jpg}
% \end{minipage}%
% \begin{minipage}{0.33\textwidth}
%     \includegraphics[width=\linewidth]{image5.jpg}
% \end{minipage}%
% \begin{minipage}{0.33\textwidth}
%     \includegraphics[width=\linewidth]{image6.jpg}
% \end{minipage}
\begin{figure}
    \centering
    \includegraphics[width=13.5cm,scale=1.0]{NeurIPS 2024/figure/heatmaps_conbias.pdf}
    \caption{\small \textbf{Top}: Attributions of base model. \textbf{Middle}: Attributions of ALIA-trained model.
\textbf{Bottom}: Attributions of our method. Our method helps the base model focus on only the relevant features in the data, and removing reliance on shortcut features, i.e. the background. \Cheng{find more examples for the all three datasets.}}
    \label{fig:heatmaps}
\end{figure}

To verify that the model indeed debiases the imbalanced concepts that our method discovers, we present GradCAM attributions of the model predictions after retraining. In Figure \ref{fig:heatmaps}, we show results on the Waterbirds dataset. While other methods frequently focus on the spurious feature (i.e. the background), our method helps the model focus only on the relevant, object level features of the data. This was the objective of our method: To upsample underrepresented concept combinations across classes in a uniform fashion, i.e. circumvent the reliance of classifiers on such spurious correlations.

\subsubsection{Scaling the number of images in $D_{aug}$}

In Table \ref{tab:main}, we commented on the fact that our method provides marginal improvement over the baselines in the COCO-GB dataset. Our hypothesis was that this was due to the low number of images in the augmented dataset. In Figure \ref{fig:cocobg}, we demonstrate the impact of adding more images to $D_{aug}$ for retraining. Clearly, our method benefits from this protocol, leading to significant differences over ALIA as we keep increasing the number of images. Note that, infinite enrichment is not recommended and has been found to be detrimental to classifier performance. This explains why, after an inflexion point, the accuracy suffers from adding more images. Similar observations have been made in \cite{dunlap2024diversify} and

\begin{figure}[h]
\centering
% Row 1
\begin{minipage}{0.5\textwidth}
    \includegraphics[width=0.6\linewidth]{NeurIPS 2024/figure/CB_Test_Accuracies.png}
\end{minipage}%
\begin{minipage}{0.5\textwidth}
    \includegraphics[width=0.6\linewidth]{NeurIPS 2024/figure/OOD_Test_Accuracies.png}
\end{minipage}%
\caption{Class-Balanced (CB) and Out-of-Distribution (OOD) test accuracies on COCO-GB: Increasing number of images in $D_{aug}$ improves performance up to a certain point (1000 images).\Cheng{adjust the ratio.}}
\label{fig:cocobg}
\end{figure}

\subsubsection{The impact of the Generative Model}
ALIA uses an InstructPix2Pix (IP2P) based generation procedure, while we use stable diffusion with a mask-inpainting procedure to make sure the objects remain consistent in the image. To ablate the effect of the generation, we present results of our method with IP2P as the generative model instead, on Waterbirds dataset, in Figure \ref{fig:ip2p} . First, we note that even with IP2P as the generative component, we are able to outperform ALIA, which suggests that it is actually the superior quality of our concept discovery method that leads to the improved results. Second, our inpainting based method outperforms our IP2P based method, which hints at interesting future work with regards to synthetic image generation. 



\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{NeurIPS 2024/figure/plot_ip2p.pdf}
    \caption{Using IP2P as the generative component on our method with the Waterbirds dataset. Our method with IP2P is still able to outperform ALIA and the base, although our generative protocol has additional benefits. Results averaged over three training runs. \Cheng{do the table, leave it here.}}
    \label{fig:ip2p}
\end{figure}

\Cheng{show some examples for 1, 2,3 4. find actually examples.}

\Cheng{add limitation section. 1) binary; 2) efficiency; }


==> section/intro_bk.tex <==
\section{Introduction}
\label{s_intro}
Over the last decade, deep learning has witnessed an unparalleled growth in the capabilities of models across a wide range of tasks, such as image classification, object detection, semantic segmentation, and so on. More recently, with the introduction of large multi-modal models, these capabilities have improved further. The lowest common denominator in all such advances lies in the ability to curate large datasets to the order of billions of data points. Consequently, models trained on such data, while demonstrating impressive performance on a wide range of tasks, have been shown to be biased in their predictions~\cite{}. These biases come in various flavours, based in texture, shape, object co-occurrence, object scale, and so on.  

In addition to exploring model biases, dataset diagnosis, or evaluating biases directly within the dataset, is particularly crucial as large datasets available today are beyond the scope of human evaluation, owing to their size and complexity. It is time-consuming and expensive to extensively annotate data manually for possible biases. Therefore, there is an urgent need for automated tools and frameworks to effectively diagnose and debias these datasets. An initial work in this direction was REVISE, which computed object statistics directly from the dataset annotations to visualize what clear spurious correlations exist, that may hinder downstream classifier performance. 
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{NeurIPS 2024/figure/fig_intro.pdf}
    \caption{\small The conventional data diagnosis and augmentation pipeline begins with an original (biased) dataset. Typical approaches include the following steps (a) Computing object statistics \cite{wang2022revise}, (b) employing diverse domain descriptions from extracted metadata \cite{dunlap2024diversify}, and (c) augmentation techniques (e.g., \cite{yun2019cutmix}, \cite{cubuk2020randaugment}). In contrast, our framework models visual data as a knowledge graph of concepts, with orange nodes representing classes and blue nodes representing concepts. This approach facilitates a systematic diagnosis of class-concept imbalances, enabling a principled method for debiasing object co-occurrences in image datasets.  }
    \label{fig:intro}
    \vspace{-6mm}
\end{figure}

More recently, the bias taxonomy for visual data has been more carefully explored. While multiple works exist in the categorization and exploration of biases in visual data~\cite{}, an end-to-end pipeline incorporating both diagnosis and debiasing has received relatively scant attention. ALIA \cite{dunlap2024diversify} is the closest and most recent work exploring such a data-augmentation-based approach to debiasing, but it has two issues - first, it does not diagnose the dataset which it aims to debias. Without such a diagnosis, it is challenging to identify the biases to be mitigated in the first place. Second, the method relies on a large language model (ChatGPT-4~\cite{gpt3}) to generate diverse, unbiased, in-domain descriptions. This is inherently problematic since relying on a large language model to debias a dataset may confound the model with inherited biases from the external model itself (in this case, ChatGPT-4). In this work, we propose to solve both of these issues. 

Our key contribution is in representing a visual dataset as a knowledge graph of concepts. Analyzing this graph for imbalanced class-concept combinations leads to a principled diagnosis of biases present in the dataset. 
Once identified, we generate images to address under-represented class-concept combinations, promoting a more uniform concept distribution across classes. 
 By using a concept graph, we circumvent the reliance on a large language model to generate debiased data. Figure~\ref{fig:intro} illustrates the core idea of our approach in contrast with existing methods. We target object co-occurrence bias, a human-interpretable issue known to confound downstream tasks \cite{oliva2007role, galleguillos2008object}. Object co-occurrence bias refers to any spurious correlation between a label and an object causally unrelated to the label.  Representing the dataset as a knowledge graph of object co-occurrences provides a structured and controllable method to diagnose and mitigate these spurious correlations.

Our framework proceeds in three steps - (1) \textbf{Concept Graph Construction:} We construct a knowledge graph of concepts from the dataset. These concepts are assumed to come from dataset ground truth (such as captions or segmentation masks). (2) {\bf Concept Diagnosis Stage:} 
This stage then analyzes the knowledge graph for concept imbalances, revealing potential biases in the original dataset. (3) {\bf Concept Debiasing Stage:} We sample imbalanced concept combinations from the knowledge graph using graph cliques, each representing a class-concept combination identified as imbalanced.  We then generate images containing under-represented concept combinations to supplement the dataset. The image generation protocol is generic and uses an off-the-shelf inpainting process with a text-to-image generative model. This principled approach ensures that the concept distribution in our augmented data is uniform and less biased. Our experiments validate this approach, showing that data augmentation based on a balanced concept distribution improves generalization performance across multiple datasets compared to existing baselines. In summary, our contributions include:

\begin{itemize}[itemsep=5pt,topsep=5pt,leftmargin=15pt]
    \item Proposing a new concept graph-based framework to diagnose biases in visual datasets. A concept graph promotes a principled approach to diagnosing datasets for biases, and to mitigating them. 

    \item  Based on the graph construction and diagnosis, we propose a novel clique-based concept balancing strategy to address detected biases.

     \item We demonstrate that balanced concept generation in data augmentation enhances classifier generalization across multiple datasets, over baselines. 
\end{itemize}

==> section/limitations.tex <==
\section{Limitations}

While ConBias is the first end-to-end pipeline to both diagnose and debias visual datasets, there are some limitations: First, that the enumeration of clique grows exponentially with the size of the graph. While we find cliques of size four to be sufficient for the datasets in this work, there could be more efficient strategies to find the concept combinations. Second, in this work we focus on biases emanating out of object co-occurrences. A variety of other biases exist in vision datasets, and future work would look to address the same. Further, we assume access to high quality annotations in the metadata. We must note, therefore, that incorrect or unreliable Finally, while the stable diffusion generation protocol leads to impressive results over baselines, more automated techniques to verify the quality of generated samples remains an interesting area of future research.

==> table/graph_structure.tex <==
\newcommand{\gup}{\textcolor{green}{$\uparrow$}} % Define the green up-arrow
\newcommand{\ourmethod}{{\sc {ConBias}}\xspace}
\begin{table}[t]
    \small
    \tabcolsep 10pt
    \centering
    \caption{\small \textbf{Multiple Shortcut Mitigation by using the graph structure.} Only computing single concept-class frequency counts does not remove reliance on both the background and co-occurring object bias. \Cheng{we will wrap this table with the text at last.}}
    \begin{tabular}{lccc}
        \toprule
        Model & CB $\uparrow$ & OOD $\uparrow$ \\
        \midrule
        Base & 73.47 & 40.47 \\
        ALIA & 74.00 & 42.53 \\
        \midrule
        Base (BG) & 78.53 & 51.93 \\
        Base (CoObj) & 77.00 & 47.30 \\
        Base (Both) & 78.13 & 51.39 \\
        Base (\ourmethod) & \textbf{79.40} & \textbf{53.20} \\
        \bottomrule
    \end{tabular}
    \label{tab:graph}
\end{table}

==> table/ip2p_acc.tex <==
\begin{table}[t]
    \centering
    \small
    \tabcolsep 8pt
    \caption{\small CB and OOD Accuracies for the IP2P variant of our model with respect to base, ALIA, and our original model. Our method significantly improves over ALIA even when using IP2P, although the best results are still achieved when using the stable diffusion based inpainting protocol.}
    \begin{tabular}{lccc}     
        \toprule
        \textbf{Models} & \textbf{CB} $\uparrow$ & \textbf{OOD} $\uparrow$ \\
        \midrule
        Base & 67.1 & 44.9 \\
        Base + ALIA & 69.6 & 48.2 \\
        \midrule
        Base + Ours (IP2P) & 72.9 & 60.48 \\
        Base + Ours & \textbf{77.9} & \textbf{69.3} \\
        \bottomrule
    \end{tabular}
    \vspace{3mm}
    \label{tab:ip2p-accuracy}
\end{table}
